Regularized Nonsmooth Newton Algorithms for Best Approximation

We consider the problem of finding the best approximation point from a polyhedral set, and its applications, in particular to solving large-scale linear programs. The classical projection problem has many various and many applications. We study a regularized nonsmooth Newton type solution method where the Jacobian is singular; and we compare the computational performance to that of the classical projection method of Halperin-Lions-Wittmann-Bauschke (HLWB). We observe empirically that the regularized nonsmooth method significantly outperforms the HLWB method. However, the HLWB has a convergence guarantee while the nonsmooth method is not monotonic and does not guarantee convergence due in part to singularity of the generalized Jacobian. Our application to solving large-scale linear programs uses a parametrized projection problem. This leads to a \emph{stepping stone external path following} algorithm. Other applications are finding triangles from branch and bound methods, and generalized constrained linear least squares. We include scaling methods that improve the efficiency and robustness.

==> dense3deg.tex <==
\begin{tabular}{|ccc||ccccc|ccccc|} \hline
\multicolumn{3}{|c||}{Specifications} & \multicolumn{5}{|c|}{Time (s)} & \multicolumn{5}{|c|}{Rel. Resids.}\cr\cline{1-13}
  $m$&   $n$& \% density&  Exact & Inexact &    HLWB &  lsqlin &   QPPAL &   Exact & Inexact &    HLWB &  lsqlin &   QPPAL \cr\hline
  300 &  1000 &   25 &3.90e-02 & 4.37e-01 & 4.58e+01 & 3.25e-01 & 2.25e+00 &  5.12e-17 & 1.23e-17 & 1.34e-04 & 9.04e-16 & -5.76e-16 \cr\hline
  300 &  1000 &   50 &6.52e-02 & 3.55e-01 & 5.42e+01 & 3.24e-01 & 1.38e+01 &  2.54e-17 & 9.84e-16 & 1.49e-04 & 6.69e-18 & -1.90e-15 \cr\hline
  300 &  1000 &   75 &9.85e-02 & 2.94e-01 & 5.32e+01 & 3.33e-01 & 5.41e+01 &  3.76e-17 & 3.06e-16 & 1.54e-04 & 3.17e-17 & 4.48e-15 \cr\hline
  300 &  1000 &  100 &1.50e-01 & 3.03e-01 & 4.79e+01 & 2.88e-01 & 2.96e+02 &  4.43e-17 & 2.01e-17 & 1.47e-04 & 1.42e-16 & -9.59e-14 \cr\hline
\end{tabular}


==> sizeM3deg.tex <==
\begin{tabular}{|ccc||ccccc|ccccc|} \hline
\multicolumn{3}{|c||}{Specifications} & \multicolumn{5}{|c|}{Time (s)} & \multicolumn{5}{|c|}{Rel. Resids.}\cr\cline{1-13}
  $m$&   $n$& \% density&  Exact & Inexact &    HLWB &  lsqlin &   QPPAL &   Exact & Inexact &    HLWB &  lsqlin &   QPPAL \cr\hline
  500 &  3000 & 8.1e-01 &4.99e-02 & 1.83e-01 & 1.54e+02 & 3.80e+00 & 2.66e+01 &  2.88e-15 & 5.37e-17 & 2.25e-04 & 8.20e-17 & 3.07e-16 \cr\hline
 1000 &  3000 & 8.1e-01 &4.64e-01 & 1.12e+00 & 3.71e+02 & 5.98e+00 & 3.63e+00 &  5.23e-18 & 4.35e-15 & 2.04e-04 & 6.42e-17 & -2.20e-16 \cr\hline
 1500 &  3000 & 8.1e-01 &3.45e+00 & 4.53e+00 & 6.14e+02 & 7.07e+00 & 8.61e+00 &  3.89e-18 & 2.28e-18 & 1.99e-04 & 2.02e-16 & 1.14e-16 \cr\hline
 2000 &  3000 & 8.1e-01 &8.22e+00 & 8.02e+00 & 8.71e+02 & 1.94e+03 & 2.88e+01 &  1.27e-16 & 9.78e-17 & 2.16e-04 & 3.94e-18 & -1.66e-16 \cr\hline
\end{tabular}


==> sizeN3deg.tex <==
\begin{tabular}{|ccc||ccccc|ccccc|} \hline
\multicolumn{3}{|c||}{Specifications} & \multicolumn{5}{|c|}{Time (s)} & \multicolumn{5}{|c|}{Rel. Resids.}\cr\cline{1-13}
  $m$&   $n$& \% density&  Exact & Inexact &    HLWB &  lsqlin &   QPPAL &   Exact & Inexact &    HLWB &  lsqlin &   QPPAL \cr\hline
  200 &  3000 & 8.1e-01 &2.52e-03 & 3.94e-02 & 4.40e+01 & 3.34e+00 & 9.36e+00 &  7.23e-18 & 2.71e-18 & 2.43e-04 & 3.53e-17 & -8.12e-16 \cr\hline
  200 &  3500 & 8.1e-01 &2.41e-03 & 3.81e-02 & 5.09e+01 & 5.16e+00 & 1.80e+01 &  2.69e-16 & 2.10e-18 & 2.70e-04 & 6.63e-16 & -1.10e-15 \cr\hline
  200 &  4000 & 8.1e-01 &3.17e-03 & 3.62e-02 & 5.87e+01 & 7.07e+00 & 1.13e+01 &  5.29e-18 & 2.77e-18 & 2.69e-04 & 4.69e-17 & 2.30e-15 \cr\hline
  200 &  4500 & 8.1e-01 &3.49e-03 & 4.17e-02 & 6.57e+01 & 9.39e+00 & 2.43e+01 &  4.94e-18 & 1.90e-18 & 3.11e-04 & 5.94e-16 & 2.94e-15 \cr\hline
\end{tabular}

